Dynamic IFC Theorems for Free!

We show that noninterference and transparency, the key soundness theorems for dynamic IFC libraries, can be obtained "for free", as direct consequences of the more general parametricity theorem of type abstraction. This allows us to give very short soundness proofs for dynamic IFC libraries such as faceted values and LIO. Our proofs stay short even when fully mechanized for Agda implementations of the libraries in terms of type abstraction.

==> Effects.tex <==
\begin{figure}
  \begin{agda}
module FacState (imp : MultefInterface) where
  open MultefInterface imp
  -- FSt Computations
  State : Set
  State = String → Bool

  FSt : Set → Set
  FSt = State → Fac (State × A)

  -- Monadic Fragment
  return : {A : Set} → A → FSt A
  return a = λ s → return (s , a)

  bind : {A B : Set} → FSt A
      → (A → FSt B) → FSt B
  bind f c = λ s → &\kw{do}&
    (s' , a) ← f
    c a s'

  lift : {A : Set} → Fac A → FSt A
  lift f = λ s → &\kw{do}&
    a ← f
    return (s , a)

  -- State Monad
  get : FSt State
  get = λ s → return (s , s)

  put : State → FSt ⊤
  put s' = λ s → return (s' , tt)

  -- Derived Operations
  read : String → FSt Bool
  read var = &\kw{do}&
    s ← get
    return (s var)
  
  write : String → Bool → FSt ⊤
  write var val = &\kw{do}&
    s ← get
    put (λ var' → &\kw{if}& var==var' &\kw{then}&
                     val
                   &\kw{else}&
                     s var')

  \end{agda}
  \caption{\label{fig:FSt} FacState implementation on top of Multef}
\end{figure}

The libraries that we have investigated so far only offer dynamic IFC
functionality for programs without side effects.
%
However, following \citet{DCCInHaskell}, we can use the old trick of
\emph{Monad Transformers} \cite{10.1145/199448.199528} to extend our current
libraries with monadic side effects.
%
In short, a monad transformer is something that can take a monad and add
extra functionality to it, while retaining the monadic structure.
%
Formally, a monad transformer is a function:
%
\begin{agda}
  T : (Set → Set) → (Set → Set)
\end{agda}
%
Such that if \ai{M : Set → Set} is a monad, then so is \ai{T M}.
%
Furthermore, \ai{T M} must retain the structure of \ai{M}, and so
there is required to be a function:
%
\begin{agda}
lift : {A : Set} → M A → T M A
\end{agda}
%
with the role of lifting \ai{M}-computations to \ai{T M} computations.

The quintessential example of a monad transformer is \ai{StateT}.
%
This monad transformer makes a monad stateful, by threading through a state of
type \ai{State} using the following transformation:
%
\begin{agda}
StateT M A = State → M (State × A).
\end{agda}
%
In other words, a \ai{StateT M A} computation is a computation that starts with
an initial state and performs some actions in \ai{M} and produces a new state
and a result \ai{A}.

\Cref{fig:FSt} shows the special case of how we can instantiate the
\ai{StateT} monad transformer with the \ai{Fac} monad to create the \ai{FSt}
monad (for ``faceted state'') .
%
The definitions of \ai{return}, \ai{bind}, and \ai{lift} are straightforward.
%
By abuse of notation, we allow the names \ai{return} and \ai{bind}, and so also
the use of \ai{do}-notation, to overlap between the \ai{M} and \ai{StateT M} monads.

On top of these mundane monadic operations, \ai{StateT} also provides
functions for accessing and updating the state in a computation, \ai{get}
and \ai{put}.
%
Furthermore, with the specific instantiation of the \ai{State} type in the
\ai{FacState} module, mapping strings to booleans, we can also define more
practical \ai{read} and \ai{write} operations to update a single mapping.

The module \ai{FacState} \emph{abstractly} depends on the \ai{MultefInterface},
and so the extension constitutes what we have previously called ``client
code''.
%
This means that we have no proof obligation for noninterference for \ai{FSt}
computations, it follows from noninterference for the \ai{sec : MultefInterface}
instantiation of the Multef interface.
%
That is, because all the code of this section treats Multef abstractly, we do
not need to define any special logical relation or proof, and can use the
standard interpretation of \cref{def:rel-types,def:rel-terms}.

The \ai{FSt} monad allows us to implement the following
canonical example for faceted state adapted from \citet{MF}:
%
\begin{agda}
example : Fac Bool → FSt Bool
example fx = &\kw{do}&
  write "y" True
  write "z" True

  x ← lift fx
  &\kw{if}& x &\kw{then}& write "y" False &\kw{else}& return tt

  y ← read "y"
  &\kw{if}& y &\kw{then}& write "z" False &\kw{else}& return tt

  z ← read "z"
  return z
\end{agda}
%

The module in \cref{fig:FSt} is parametric in the implementation
\ai{imp : MultefInterface} of the faceted library.
%
One only obtains actual runnable code by linking this module with
the implementation of \ai{MultefInterface} one is interested in. 
%
Naturally, whatever guarantees are provided by that implementation will
then be inherited by the resulting \ai{FacState imp} module.
%
This means that noninterference for \ai{FacState sec} follows automatically
from noninterference for \ai{sec : MultefInterface}.
%

\ifsooner
\jpb{In the mechanization, the proof of non-interference relies on
  StateT satisfying identity extension. That is \ai{[[StateT]] _≡_} is the
  identity. And so, the proof goes through for every functor, because
  they all have this property (proof relies on parametricity + the
  functor laws and is standard.)}
\ma{That's actually really cool! Had we had more time I would have said let's
write a chapter about it. As it is right now, I'm hesitant to re-organize much.
Though we will get much more extra space if we get accepted...}

\todo{Talk briefly about other effects as well, not just state}
\ma{Specifically, we should probably talk about exceptions as monad transformers, they are important}
\ch{I would intuitively expect exceptions to be special, so they had to be baked
  into our core calculus, and that one wouldn't get the same thing by just
  applying a monad transformer. Probably worth investigating anyway though.}
\fi


==> agda-primer.tex <==
%\subsection{Quick Primer to Agda Syntax} ma: Orphaned subsection.




==> app-agda-port.tex <==
\begin{figure}
  \begin{agda}
record LIOInterface : Set₁ where
  field
    -- Labeled Values
    Labeled   : Set → Set
    label     : {A : Set} → Label → A → Labeled A
    labelOf   : {A : Set} → Labeled A → Label
    -- LIO Computations
    LIO       : Set → Set
    return    : {A : Set} → A → LIO A
    bind      : {A B : Set} → LIO A
             → (A → LIO B) → LIO B
    unlabel   : {A : Set} → Labeled A → LIO A
    toLabeled : {A : Set} → Label
             → LIO A → LIO (Labeled A)
    -- Exceptions
    throw     : {A : Set} → UserError → LIO A
    catch     : {A : Set} → LIO A
             → (E → LIO A) → LIO A


sec : LIOInterface
sec = { -- Labeled Values
        Labeled A       = (A ⊎ E) × Label
      ; label ℓ a       = inj₁ a , ℓ
      ; labelOf (a , ℓ) = ℓ
      -- LIO Computations
      ; LIO A = (ℓc : Label) →
              Σ ((A ⊎ E) × Label)
              (λ { (r , ℓc') → ℓc ⊑ ℓc' })
      ; return a ℓc = (inj₁ a , ℓc) , ⊑-refl
      ; bind lio cont ℓc = case (lio ℓc) of
          ((inj₁ a , ℓc') , pr) →
            let r , pr' = cont a ℓc' in
            (r , ⊑-trans pr pr')
          ((inj₂ e , ℓc') , pr) → (inj₂ e , ℓc') , pr
      ; unlabel (r , ℓ) ℓc =
          ( (r , ℓ ⊔ ℓc)
          , ⊑-trans ⊔-mono (⊑-eql ⊔-comm))
      ; toLabeled ℓ lio ℓc =
          let ((r , ℓc') , pr) = lio ℓc in
          if ℓc' ⊑ ℓ then
            ((inj₁ (r , ℓ) , ℓc) , ⊑-refl)
          else
            (inj₁ (inj₂ (EIFC (ToLabeledError ℓ) ℓc) , ℓ) , ℓc)
            , ⊑-refl
      -- Exceptions
      ; throw e ℓc = (inj₂ (EUser e ℓc) , ℓc), ⊑-refl
      ; catch lio hnd ℓc = case (lio ℓc) of
          (inj₁ a , ℓc') , pr → (inj₁ a , ℓc') , pr
          (inj₂ e , ℓc') , pr →
            let c , pr' = hnd e ℓc' in
            (c , ⊑-trans pr pr')
      }
  \end{agda}
  \caption{\label{fig:lio} Our Agda port of the core LIO library}
\end{figure}


==> embedding.tex <==
\jpb{This section can be deleted, or put in appendix for pedantry.}
\begin{figure}
\begin{align*}
  t ::=&\ \star\ |\ \square\ |\ x\ |\ (x : t) \to t\ |\ \lambda x : t.\ t\\
      |&\ t\ t\ |\ \record\{\many{n : t}\}\ |\ \{\many{n = t}\}\ |\ t.n
\end{align*}
\caption{\label{fig:cc} The Syntax of the Calculus of Constructions
  augmented with records.}
\end{figure}

\todo{Motivate the choice to do the formal work in CC, it's simply
the easiest model that is not far removed from Agda for which we have
an easy to understand parametricity theory}

We will embed both Core Multef above and Core LIO in the Calculus of
Constructions (\CC{}) \cite{CC}
with sigma types (and record syntax).
%
The syntax of this variant of \CC{} is presented in \cref{fig:cc}.
%
Most of the constructs are standard, $\star$ is the sort of types, $\square$ of kinds,
variables are denoted by $x$, and abstraction and application use the standard syntax.
%
We eschew the $\Pi(x : A)B$ syntax for dependent product types, in favour of
the form more familiar to users of dependently typed functional languages like
Agda \cite{Agda}, namely $(x : A) \to B$.
%
Similarly, we also eschew the traditional syntax for the dependent sum, or $\Sigma$, types,
for which we adopt a record-like syntax.
%
The term $\record\{\many{n : t}\}$, where $\many{n : t} = n_1 : t_1 ; \ldots ; n_i : t_i$
represents zero or more instances of the form $n : t$, where $n$ is a field name
with type $t$.
%
We use the syntactic form $\{\many{n = t}\}$ to construct records and $t.n$ to
access the field $n$ in record $t$.

The difference between traditional record types and $\Sigma$ types is that each
field is accessible by a name $n$.
%
Because we will not use subtyping in this paper the difference
is of convenience rather than fundamental.
%
We refer to the work of \citet{10.5555/184757} for an extended discussion.
%
We further assume that field labels, $n$, are unique for any given record and
record types, avoiding any ambiguity.

Both of our embeddings will use the notion of data abstraction of
\citet{cardellimodules}.
%
\todo{Questionable citation / sentence}
%
Under this scheme, the interface of a module is encoded as a record,
and its implementation is an inhabitant of such type.
%
In particular, (abstractly) exported type is found as an abstract type
in the record type of the module, which corresponds to an existential quantification.
%
For example, consider the \ai{MultefInterface} record type from \cref{fig:multef}:
%
\begin{agda}
record MultefInterface : Set1 where
  field
    Fac    : Set -> Set
    facet  : {A : Set} -> Label -> Fac A
           -> Fac A -> Fac A
    return : {A : Set} -> A -> Fac A
    bind   : {A B : Set} -> Fac A
           -> (A -> Fac B) -> Fac B
\end{agda}
%

\begin{figure}
  \begin{alignat*}{5}
    &\mathrlap{\Multef : \square} \\
    &\Multef =&&\ \record\{\ &&\textit{Fac}    &&:\ \star \to \star;\\
    &         &&             &&\textit{facet}  &&:\ (A : \star) \to \L \to \textit{Fac}\ A \to\\
    &         &&             &&                &&\ \ \ \ \ \textit{Fac}\ A\ \to \textit{Fac}\ A;\\
    &         &&             &&\textit{return} &&:\ (A : \star) \to A\ \to \textit{Fac}\ A;\\
    &         &&             &&\textit{bind}   &&:\ (A, B : \star) \to \textit{Fac}\ A \to\\
    &         &&             &&                 &&\ \ \ \ \ (A \to \textit{Fac}\ B) \to \textit{Fac}\ B\}
  \end{alignat*}
  \begin{alignat*}{5}
    &\mathrlap{sec : \Multef} \\
    &sec =&&\ \{\ &&\textit{Fac}    &&=\ &&\lambda A : \star.\ \L \to A;\\
    &     &&      &&\textit{facet}  &&=\ &&\lambda A : \star.\lambda \ell : \L.\lambda f_0, f_1 : \textit{Fac}\ A.\lambda \ell' : \L.\\
    &     &&      &&                &&   &&\textit{if}\ \ell \canFlowTo \ell'\ \textit{then}\ f_0\ \ell'\ \textit{else}\ f_1\ \ell';\\
    &     &&      &&\textit{return} &&=\ &&\lambda A : \star.\lambda a : A.\lambda \ell : \L.\ a;\\
    &     &&      &&\textit{bind}   &&=\ &&\lambda A, B : \star.\lambda f : \textit{Fac}\ A.\\
    &     &&      &&                &&   &&\lambda c : (A \to \textit{Fac}\ B).\\
    &     &&      &&                &&   &&\lambda \ell : \L.\ c\ (f\ \ell)\ \ell\}
  \end{alignat*}
  \caption{\label{fig:cc:multef} Core Multef in \CC{}}
\end{figure}

Using the encoding of modules as records, we get the $\CC$ type $\Multef$
in \cref{fig:cc:multef}.
%
The implementation of this module corresponds to a value $m : \Multef$
and one implementation is given in \cref{fig:cc:multef}.\ch{Does this correspond
  to the one from Section 2?}
%
Accordingly, importing the $\Multef$ library corresponds to taking an
implementation of $\Multef$ as an argument.
%
More concretely, the client code in \cref{fig:Temp} can be modelled as
a parameterised record, whose type can be written in $\CC$ as follows
%
\begin{alignat*}{3}
  &\mathrlap{\textit{Temp} : \Multef \to \square}\\
  &\textit{Temp} =\ &&\mathrlap{\lambda\ m : \Multef.}\\
  &                 &&\record\{\ && \textit{HotOrCold} : \star;\\
  &                 &&           && \textit{isCold} : m.\textit{Fac}\ \textit{Int} \to m.\textit{Fac}\ \textit{HotOrCold}\}
\end{alignat*}
%
And, an implementation $\mathit{temp} : (m : \Multef) \to \textit{Temp}\ m$ that 
abstracts over the particular implementation $m : \Multef$ of the
$\Multef$ library.
%
This abstraction is important, because the implementation of $\mathit{temp}$ is
agnostic of the particular implementation of $\Multef$ it is linking to.

This abstraction is what allows us to provide IFC guarantees for the
$\textit{Temp}$ module.
%
This is done without adding any primitive to \CC, nor modifying its semantics
nor its type system.


==> future-work.tex <==
In this paper, our security libraries have been expressed directly
in the rich dependently typed language Agda.
%
Agda is similar to Haskell, the usual host language for these libraries,
in many ways.
%
However, one important feature lacking from Agda but present in Haskell
is non-termination.

Depending on your perspective, this discrepancy may or may not be worrying.
%
For example, it's reasonable to expect that introducing non-termination does
not introduce additional channels for information leakage other than the usual
termination channel, making our noninterference guarantees
termination \emph{insensitive} \cite{hedin2012perspective}.
%
However, there are Haskell security libraries that provide termination \emph{sensitive}
security guarantees \cite{stefan2012addressing}.
%
Reasoning directly about such libraries requires developing new parametricity theories
for richer languages, a task where the Iris framework may be of use \cite{jung2015iris}.


==> library-based.tex <==
\begin{figure}
  \centering
\begin{haskell}
module Multef (Fac, facet, return, (>>=)) where
import Label

data Fac a = Raw a
           | Facet Label (Fac a) (Fac a)

facet :: Label -> Fac a -> Fac a -> Fac a
facet = Facet

instance Monad Fac where
  return = Raw
  Raw a >>= k = k a
  Facet l f0 f1 >>= k = Facet l (f0 >>= k) (f1 >>= k)
\end{haskell}
  \caption{\label{fig:multef} Core Multef}
\end{figure}

Traditional library-based IFC systems like MAC \cite{MAC}
and LIO \cite{LIO} are based on one simple idea.
%
In order to ensure security, these libraries provide an interface to the IO
capabilities of the host programming language that is used by the client to
interact with the real world.
%
In order to ensure security it is not sufficient to control what IO
a program can do, it is also necessary to account for the way that information
flows within a program.
%
\todo{This bit clearly needs to be extended somewhat to make sense}

\todo{The order in this section is all messed up + making it clear what is happening in bind
etc. are completely missing}

\ch{Do we really need to call the type of facets \hsi{Fac}?
  How about \hsi{Fct} instead?}
\ma{This has never been a problem before (\cite{FSME, OptimisingFSME}), so why change it?}

Figure~\ref{fig:multef} contains the core
faceted value syntax and semantics~\cite{MF,austin2014typed}
from the Multef~\cite{FSME} library.\ch{mention that this is Haskell code}
%
A faceted value \hsi{v :: Fac a} is either a raw value \hsi{v'} of type \hsi{a},
(\IE \hsi{v = Raw v'}),
or a node containing a label \hsi{l :: Label} and two
faceted values \hsi{f0} and \hsi{f1} of type \hsi{Fac a}
(\IE \hsi{v = Facet l f0 f1}).
%
A faceted value may be a different value depending on who is observing it.
%
For example, the faceted value \hsi{Facet Alice (Raw 0) (Raw 1)} looks like
\hsi{0} to anyone who is able to observe values with \hsi{Alice}'s
confidentiality level, and looks like $1$ to everyone else.

Combining two faceted values also yields a faceted value.
%
For example, if we add \hsi{f0 = Facet Alice (Raw 0) (Raw 1)} and \hsi{f1 = Facet Bob (Raw 2) (Raw 3)}, we 
get the \emph{recursive} faceted value:
%
\begin{haskell}
f0 + f1 = Facet Alice
            (Facet Bob (Raw (0 + 2)) (Raw (0 + 3)))
            (Facet Bob (Raw (1 + 2)) (Raw (1 + 3)))
\end{haskell}
%
By inspecting this value, we see that if the observer can observe \emph{both} \hsi{Alice}'s and
\hsi{Bob}'s data, they observe the sum of \hsi{f0 + f1} as \hsi{0 + 2},
whereas an observer who can see only \hsi{Bob}'s data, \emph{not}
\hsi{Alice}'s, sees the sum as \hsi{1 + 2}.

Providing this addition operation could be done in one of two ways, either we define
addition of faceted values directly, or we provide a general computational tool on top
of which we can easily define operations like addition.
%
Clearly, the second option is favourable and so following the literature on
faceted values \cite{FSME,austin2014typed} show that faceted values form a
so-called \emph{Monad} \cite{wadler1995monads}.
%
A Monad \hsi{M} is a type former, like \hsi{Fac}, with two associated operations,
\hsi{return :: a -> M a} that takes a pure value and turns it into a monadic
value, and \hsi{(>>=) :: M a -> (a -> M b) -> M b} (pronounced ``bind'') that
takes a computation \hsi{m :: M a} and a continuation \hsi{c :: a -> M b}
and produces a computation \hsi{m >>= c :: M b}.
%
Using the monad operations, we can define addition and similar operations for
\hsi{Fac} easily in the following manner:
%
\begin{haskell}
(+) :: Fac Int -> Fac Int -> Fac Int
fx + fy = fx >>= \ x -> 
          fy >>= \ y ->
          return (x + y)
\end{haskell}
%

\todo{Talk about do-syntax here and clean up the example above. This will be worth
it for future examples}

\todo{Talk about the implementation of the monad interface for Fac, talk very
briefly about type-classes (``they are like Java interfaces'')}

In general, following the IFC literature \cite{sabelfeld2003language}, we
require the type \hsi{Label} to encode a join-semi
lattice with order \hsi{canFlowTo :: Label -> Label -> Bool} and least upper
bound (or join) \hsi{lub :: Label -> Label -> Label}.
%
Using this lattice structure, we can formally define what we mean by a value
of type \hsi{Fac a} to ``look like'' something to an observer.
%
To do this we define the following function:
%
\begin{haskell}
project :: Fac a -> Label -> a
project (Raw a) l        = a
project (Facet l' f0 f1) l =
  if l' `canFlowTo` l then
    project f0 l
  else
    project f1 l
\end{haskell}

From the definition of \hsi{project}, we can define what it means for a
program, e.g. \hsi{p :: Fac Int -> Fac Int}, to be secure.
%
The program \hsi{p} is noninterferent if given any level \hsi{l :: Label}
and two faceted values
\hsi{f0, f1 :: Fac Int} such that \hsi{project f0 l == project f1 l} we have that
\hsi{project (p f0) l == project (p f1) l}.
%
In other words, \hsi{p} does not reveal information from a different security
level to \hsi{l}.

\begin{figure}
\begin{haskell}
module Temp where

import Multef 

data HotOrCold = Hot | Cold

isCold :: Fac Int -> Fac HotOrCold
isCold fint = do
  x <- fint
  if x > 25 then
    return Hot
  else
    return Cold
\end{haskell}
  \caption{\label{fig:Temp} A Client Library for the Multef Module}
\end{figure}

To see an example of this in action, consider the \hsi{Temp} client module in Figure \ref{fig:Temp}.
%
When we give \hsi{isCold} the arguments \hsi{f0} and \hsi{f1} defined as:
%
\begin{haskell}
f0, f1 :: Fac Int
f0 = Facet Alice (Raw 10) (Raw 0)
f1 = Facet Alice (Raw 30) (Raw 0)
\end{haskell}
%
we get that:
%
\begin{haskell}
isCold f0 = Facet Alice (Raw Cold)
                        (Raw Cold)
  
isCold f1 = Facet Alice (Raw Hot)
                        (Raw Cold)
\end{haskell}
%
If the observer level \hsi{l} is \hsi{Bob}, who cannot see \hsi{Alice}'s data
(\IE \hsi{Bob `canFlowTo` Alice == False}) we have that
\hsi{project f0 Bob == project f1 Bob == 0} and also
\hsi{project (isCold f0) Bob == project (isCold f1) Bob}.

\begin{figure}
\begin{haskell}
module Bad where

import Multef 

isAlicePositive :: Fac Int -> Fac Bool
isAlicePositive (Facet Alice (Raw n) f) = Raw (n > 0)
isAlicePositive f = Raw False
\end{haskell}
  \caption{\label{fig:Bad} An Illbehaved Client Library}
\end{figure}

The goal of library based IFC is, naturally, to ensure that all client code
behaves in the same secure way as \hsi{isCold}.
%
However, suppose that we write the code in \cref{fig:Bad}.
%
The function \hsi{isAlicePositive} checks if its faceted input is precisely on
the form \hsi{Facet Alice (Raw n) f}, for some \hsi{n} and \hsi{f}, and if so
returns a raw (un-)faceted value \hsi{Raw (n > 0)} and returns \hsi{Raw False}
otherwise.
%
Unfortunately, \hsi{isAlicePositive} clearly does not have the property that if
\hsi{project f0 l} is equal to \hsi{project f1 l} then so are
\hsi{project (isAlicePositive f0) l} and \hsi{project (isAliceNegative f0) l},
and so this function is not secure.

Fortunately, however, Haskell does not allow us to write this program.
%
If we type-check the module in \cref{fig:Bad}, we get the following
type error:
%
\begin{verbatim}
Bad.hs:6:18: error:
    Not in scope: data constructor ‘Facet’
Bad.hs:6:31: error:
    Not in scope: data constructor ‘Raw’
\end{verbatim}
%
This is because the constructors \hsi{Facet} and \hsi{Raw} of the \hsi{Fac}
datatype are hidden by the Multef module.
%
Consequently, client modules are forced to use only the interface to \hsi{Fac}
that's exported by the Multef module, namely \hsi{facet},
\hsi{return}, and \hsi{(>>=)}.
%
By ensuring that these operators, combined with the other language features of the
host language, preserve the \emph{relational} invariant that all functions are secure,
we ensure that all code that depends on the Multef module is secure.
%
In \cref{sec:NIproofs} we make this reasoning precise and use it to prove noninterference
for both our Multef variant and the more involved LIO DIFC library.


==> parametricity.tex <==
%
\begin{figure}
\begin{alignat*}{2}
  \rel{\square}\                 &=\ &&\lambda A_0, A_1 : \square.\ A_0 \to A_1 \to \square\\[2mm]
  \rel{\star}\                   &=\ &&\lambda A_0, A_1 : \star.\ A_0 \to A_1 \to \star\\[2mm]
  \rel{(x : A) \to B}\           &=\ &&\lambda f_0 : (x_0 : A_0) \to B_0.\\
                                 &   &&\lambda f_1 : (x_1 : A_1) \to B_1.\\
                                 &   &&(x_0 : A_0) \to (x_1 : A_1) \to\\
                                 &   &&(R_x : \rel{A}\ x_0\ x_1) \to\\
                                 &   &&\rel{B}\ (f_0\ x_0)\ (f_1\ x_1)\\[2mm]
  \rel{\record\{\many{n : t}\}}\ &=\ &&\lambda m_0 : \record\{\many{n : t_0}\}.\lambda m_1 : \record\{\many{n : t_1}\}.\\
                                 &   &&\record\{\many{R_n : \rel{t}\ m_0.n\ m_1.n}\}\\[2mm]
  \rel{\{\many{n = t}\}}\        &=\ &&\{\many{R_n = \rel{t}}\}\\[2mm]
  \rel{t.n}\                     &=\ &&\rel{t}.R_n\\[2mm]
  \rel{t\ a}\                    &=\ &&\rel{t}\ a_0\ a_1\ \rel{a}\\[2mm]
  \rel{\lambda x : A.\ b}\       &=\ &&\lambda x_0 : A_0.\ \lambda x_1 : A_1.\ \lambda R_x : \rel{A}\ x_0\ x_1.\ \rel{b}\\[2mm]
  \rel{x}\                       &=\ &&R_x
\end{alignat*}
  \caption{\label{fig:rel-cc} The Relational Translation of \CC~terms.}
\end{figure}

\todo{We need to provide intuition before diving into the technical details here}

The parametricity theory for the Calculus of Constructions, developed
by \citet{ParametricityJFP} consists of two parts.
%
First, it defines a meta-level function
translating a term in \CC{} to another term in \CC{}:
%
$$
\rel{\_} : \text{\CC} \to \text{\CC}
$$
%
%
Second, it gives a fundamental (meta)theorem, parametricity, that relates
well-typedness of expressions and the translation:
%
\begin{proposition}[Parametricity]
  \label{prop:parametricity}
  If $\vdash e : t$ then $\vdash \rel{e} : \rel{t}\ e\ e$.
\end{proposition}
%
Loosely speaking, if $t$ is a type, then $\rel{t} : t \to t \to \star$ is
a relation on types, and if $e : t$ is a term, then $\rel{e} : \rel{t}\ e\ e$
is a proof that $e$ is related to itself by the relation $\rel{t}$.

The definition of $\rel{\_}$ can be found in \cref{fig:rel-cc}.
%
To see how the translation of types works, consider the following example
type for the parametrically polymorphic ``const'' function:
%
$$
(A\ B : \star) \to A \to B \to A
$$
%
We are going to prove something close to ``noninterference'' for any function $f$
of this type.
%
Namely, we are going to show that given any $A$ and $B$, $a : A$ and any two $b_0, b_1 : B$,
it is the case that $f\ A\ B\ a\ b_0 \equiv f\ A\ B\ a\ b_1$.

Intuitively, this is true because $f$ needs to be able to work with \emph{any} types
$A$ and $B$.
%
Absent any other information than that $A$ and $B$ are types respectively,
there is nothing the implementor of $f$ can do with a value of type $B$ to
influence the output at type $A$.
%
Next we will make this intuitive reasoning precise by appealing to parametricity.

From the definition in \cref{fig:rel-cc} we can compute the relation associated
with the type above as:
%
\begin{align*}
  &\rel{(A\ B : \star) \to A \to B \to A} =\\
  &\ \ \ \lambda f_0, f_1 : (A\ B : \star) \to A \to B \to A.\\
  &\ \ \ (A_0 : \star) \to (A_1 : \star) \to (R_A : A_0 \to A_1 \to \star) \to\\
  &\ \ \ (B_0 : \star) \to (B_1 : \star) \to (R_B : B_0 \to B_1 \to \star) \to\\
  &\ \ \ (a_0 : A_0) \to (a_1 : A_1) \to (R_a : R_A\ a_0\ a_1) \to\\
  &\ \ \ (b_0 : B_0) \to (b_1 : B_1) \to (R_b : R_B\ b_0\ b_1) \to\\
  &\ \ \ R_A\ (f_0\ A_0\ B_0\ a_0\ b_0)\ (f_1\ A_1\ B_1\ a_1\ b_1)
\end{align*}
%
While this looks complicated, breaking it down reveals that the statement
makes intuitive sense.
%
Two functions $f_0\ f_1 : (A\ B : \star) \to A \to B \to A$ are related
at $\rel{(A\ B : \star) \to A \to B \to A}$ if:
%
\begin{enumerate}
  \item Given two types $A_0\ A_1 : \star$ with a relation $R_A$ between them, and
  \item two types $B_0\ B_1 : \star$ with a relation $R_B$ between them, and
  \item two elements $a_0 : A_0$ and $a_1 : A_1$ that are related by $R_A$, and
  \item two elements $b_0 : B_0$ and $b_1 : B_1$ that are related by $R_B$, we have that
  \item the results of $f_0\ A_0\ B_0\ a_0\ b_0$ and $f_1\ A_1\ B_1\ a_1\ b_1$ are related
    by $R_A$.
\end{enumerate}
%
\todo{It is difficult to make it intuitive because we always have two \emph{different} types $A_0$ $A_1$ instead of
just having $A$ and $R_A : A \to A \to \star$. I don't know how to get around this issue presentation-wise, because
for everything to actually work out we really do need two different types. However, I don't know how to intuitively
explain this \emph{when it comes to types} until we are talking about two different types introduced by two different
modules (i.e. in the transparency proof)}
%
\todo{The intuitive bit...}

The statement we want to prove is:
%
\begin{align*}
  &\forall f : (A\ B : \star) \to A \to B \to A.\\
  &\forall A\ B : \star.\ \forall a : A.\ \forall b_0\ b_1 : B.\\
  &f\ A\ B\ a\ b_0 \equiv f\ A\ B\ a\ b_1
\end{align*}
%
Given an $f : (A\ B : \star) \to A \to B \to A$, parametricity tells us that:
%
\begin{align*}
  \rel{f} &:   (A_0, A_1 : \star) \to (R_A : A_0 \to A_1 \to \star)\\
          &\to (B_0, B_1 : \star) \to (R_B : B_0 \to B_1 \to \star)\\
          &\to (a_0 : A_0) \to (a_1 : A_1) \to (R_a : R_A\ a_0\ a_1)\\
          &\to (b_0 : B_0) \to (b_1 : B_1) \to (R_b : R_B\ b_0\ b_1)\\
          &\to R_A\ (f\ A_0\ B_0\ a_0\ b_0)\ (f\ A_1\ B_1\ a_1\ b_1)
\end{align*}
%
For any two $A\ B : \star$, we have that:
%
\begin{alignat*}{2}
  \mathrlap{\rel{f}\ A\ A\ \equiv_A\ B\ B\ (\lambda b_0\ b_1 : B.\ \top) :}\\
          &           &&\ (a_0\ a_1 : A) \to (R_a : a_0 \equiv_A a_1)\\
          &\ \ \ \ \to&&\ (b_0\ b_1 : B) \to (R_b : \top)\\
          &\ \ \ \ \to&&\ f\ A\ B\ a_0\ b_0 \equiv_A f\ A\ B\ a_1\ b_1
\end{alignat*}
%
Where $\equiv_A$ is propositional equality, and $\top$ is the
one element type with $() : \top$ often called ``unit''.
%
This means that, for any $a : A$ and $b_0\ b_1 : B$, we have:
%
\begin{align*}
  &\rel{f}\ A\ A\ \equiv_A\ B\ B\ (\lambda b_0\ b_1 : B.\ \top)\ a\ a\ (\textit{refl}\ A\ a)\ b_0\ b_1\ ()\ :\\
  &\ \ \ \ f\ A\ B\ a\ b_0 \equiv_A f\ A\ B\ a\ b_1
\end{align*}
%
Where $\textit{refl} : (A : \star) \to (a : A) \to a \equiv_A a$ is the witness
of reflexivity of propositional equality.
%
In other words, from $\rel{f}$ we have derived the proof that $f$ is invariant to
its second argument.
%
\todo{We need an intuitive explanation of what is going on here!}


The final piece of the puzzle we need to understand in order to make
sense of the parametricity theory is to see how $\rel{\_}$ acts on terms.
%
Recall, each closed term $f : t$ translates to a proof $\rel{f} : \rel{t}\ f\ f$.
%
To see how this works, examine the standard definition of the constant function,
$const = \lambda A\ B : \star.\ \lambda a : A.\ \lambda b : B.\ a$ and its translation:
%
\begin{align*}
     &\rel{\lambda A\ B : \star.\ \lambda a : A.\ \lambda b : B.\ a}\\
  =\ &\lambda A_0, A_1 : \star.\ \lambda R_A : A_0 \to A_1 \to \star.\\
     &\rel{\lambda B : \star.\ \lambda a : A.\ \lambda b : B.\ a}\\
  =\ &\lambda A_0, A_1 : \star.\ \lambda R_A : A_0 \to A_1 \to \star.\\
     &\lambda B_0, B_1 : \star.\ \lambda R_B : B_0 \to B_1 \to \star.\\
     &\rel{\lambda a : A.\ \lambda b : B.\ a}\\
  =\ &\lambda A_0, A_1 : \star.\ \lambda R_A : A_0 \to A_1 \to \star.\\
     &\lambda B_0, B_1 : \star.\ \lambda R_B : B_0 \to B_1 \to \star.\\
     &\lambda a_0 : A_0.\ \lambda a_1 : A_1.\ \lambda R_a : R_A\ a_0\ a_1.\\
     &\rel{\lambda b : B.\ a}\\
  =\ &\lambda A_0, A_1 : \star.\ \lambda R_A : A_0 \to A_1 \to \star.\\
     &\lambda B_0, B_1 : \star.\ \lambda R_B : B_0 \to B_1 \to \star.\\
     &\lambda a_0 : A_0.\ \lambda a_1 : A_1.\ \lambda R_a : R_A\ a_0\ a_1.\\
     &\lambda b_0 : B_0.\ \lambda b_1 : B_1.\ \lambda R_b : R_B\ b_0\ b_1.\\
     &\rel{a}\\
  =\ &\lambda A_0, A_1 : \star.\ \lambda R_A : A_0 \to A_1 \to \star.\\
     &\lambda B_0, B_1 : \star.\ \lambda R_B : B_0 \to B_1 \to \star.\\
     &\lambda a_0 : A_0.\ \lambda a_1 : A_1.\ \lambda R_a : R_A\ a_0\ a_1.\\
     &\lambda b_0 : B_0.\ \lambda b_1 : B_1.\ \lambda R_b : R_B\ b_0\ b_1.\\
     &R_a\\
\end{align*}

\todo{Make sure modules have been introduced before this point (not their parametricity,
just how they work)}

Now that we have seen how parametricity works for ordinary functions, we will
see how it can be used to prove properties about types and their interfaces.
%
Consider the simple module:
%
\begin{alignat*}{2}
  &\mathrlap{\textit{Booleans} : \square}\\
  &\textit{Booleans} = \record\{\ &&\Bool  : \star;\\
                                & &&\true  : \Bool;\\
                                & &&\false : \Bool;\\
                                & &&\wedge : \Bool \to \Bool \to \Bool\}
\end{alignat*}
%
It exports a type, $\Bool$, two constants $\true$ and $\false$ of type $\Bool$,
and an operation $\wedge : \Bool \to \Bool \to \Bool$.
%
Unsurprisingly, there are many ways of instantiating this module, but let us simply
instantiate it in what one may consider the standard way:
%
\begin{alignat*}{2}
  &\mathrlap{\textit{booleans} : \textit{Booleans}}\\
  &\textit{booleans} = \{\ &&\Bool = \top + \top;\\
                         & &&\true = \inl\ ();\\
                         & &&\false = \inr\ ();\\
                         & &&\wedge = \lambda a\ b : \top + \top.\ \textit{case}\ a\ \textit{of}\\
                         & &&\ \ \ \ \ \ \ \ \ \ \inl\ () = b\\
                         & &&\ \ \ \ \ \ \ \ \ \ \inr\ () = \inr\ ()\}
\end{alignat*}
%
What may be surprising about the $\textit{Booleans}$ module is that
when we use it, we always end up writing monotonic functions.
%
More precisely speaking, if you write a function
$o : (imp : \textit{Booleans}) \to imp.\Bool \to imp.\Bool$,
it is straightforward to prove, using parametricity, that
if $b_0\ b_1 : \top + \top$ are two booleans such that $b_0$
implies $b_1$ then $o\ \textit{booleans}\ b_0$
implies $o\ \textit{booleans}\ b_1$.
%
One can understand why, intuitively, this is true by considering
the simple fact that the $\textit{Booleans}$ interface gives the
$o$ function no way to do negation.
%
This means that all $o\ imp$ can do to its $b : imp.\Bool$ argument is
to either discard it and return either $imp.\true$ or $imp.\false$,
or take the conjunction of some number of constants and $b$.
%
Finally, $o\ imp$ can also call other functions that are parametric in
$imp$.
%
However, ``by induction'', these functions are also monotonic.

The above argument is woefully informal, and the appeal to ``induction''
is imprecise.
%
However, parametricity is all about ``automatically'' pinning down these kinds
of arguments.
%
To see how this works formally, we need to understand two things.
%
Firstly, $\rel{\textit{Booleans}}$ tells us how to relate two implementations
of $\textit{Booleans}$:
%
\begin{alignat*}{4}
  &\mathrlap{\rel{\textit{Booleans}} : \textit{Booleans} \to \textit{Booleans} \to \square}\\
  &\mathrlap{\rel{\textit{Booleans}}\ m_0\ m_1=}\\
  &\ \ \ \record\{\ &&R_\Bool  &&\ :&&\ m_0.\Bool \to m_1.\Bool \to \star;\\
  &                 &&R_\true  &&\ :&&\ R_\Bool\ m_0.\true\ m_1.\true;\\
  &                 &&R_\false &&\ :&&\ R_\Bool\ m_0.\false\ m_1.\false;\\
  &                 &&R_\wedge &&\ :&&\ (a_0 : m_0.\Bool) \to (a_1 : m_1.\Bool)\\
  &                 &&          &&\to&&\ (R_a : R_\Bool\ a_0\ a_1)\\
  &                 &&          &&\to&&\ (b_0 : m_0.\Bool) \to (b_1 : m_1.\Bool)\\
  &                 &&          &&\to&&\ (R_b : R_\Bool\ b_0\ b_1)\\
  &                 &&          &&\to&&\ R_\Bool\ (a_0\ m_0.\wedge\ b_0)\ (a_1\ m_1.\wedge\ b_1)\}
\end{alignat*}
%
We can combine this with $\rel{o}$:
%
\begin{alignat*}{2}
  \rel{o} &\ :&&\ (imp_0\ imp_1 : \textit{Booleans})\\
          &\to&&\ (R_{imp} : \rel{\textit{Booleans}}\ imp_0\ imp_1)\\
          &\to&&\ (b_0 : imp_0.\Bool) \to (b_1 : imp_1.\Bool)\\
          &\to&&\ (R_b : R_{imp}.R_\Bool\ b_0\ b_1)\\
          &\to&&\ R_{imp}.R_\Bool\ (o\ imp_0\ b_0)\ (o\ imp_1\ b_1)
\end{alignat*}
%
And all it takes to prove our theorem is to realise that:
%
\begin{enumerate}
  \item We care about two $\textit{booleans}.\Bool$, so $imp_0 = imp_1 = \textit{booleans}$, and
  \item $R_{imp} : \rel{\textit{Booleans}}\ \textit{booleans}\ \textit{booleans}$ is an argument that
    we get to pick, and
  \item the final thing we want to prove is that if $b_0 \implies b_1$, then $o\ \ldots\ b_0 \implies o\ \ldots\ b_1$,
    so we want $R_{imp}.R_\Bool\ b_0\ b_1 = b_0 \implies b_1$.
\end{enumerate}
%
With insight (2) and (3) we can straightforwardly define $R_{imp}$ as:
%
\begin{alignat*}{3}
  &\mathrlap{R_{imp} : \rel{\textit{Booleans}}\ \textit{booleans}\ \textit{booleans}}\\
  &R_{imp}= \{\ &&R_\Bool  &&=\ \implies;\\
  &             &&R_\true  &&=\ \ldots;\\
  &             &&R_\false &&=\ \ldots;\\
  &             &&R_\wedge &&=\ \ldots\}
\end{alignat*}
%
\todo{I don't know why this typesets weirdly and how to fix it. I hate alignat}
%
Where the encoding of $\implies$ and the respective proofs, $R_\true$ that $\true \implies \true$,
$R_\false$ that $\false \implies \false$, and $R_\wedge$ that $a_0 \implies a_1$ and $b_0 \implies b_1$
gives that $a_0 \wedge b_0 \implies a_1 \wedge b_1$ are all somewhat tedious but straightforward
and can be found in the agda mechanisation.
%
\todo{Make sure to add this to the mechanisation}

Now, suppose we added negation to the interface of $\textit{Booleans}$, with the usual definition in
$\textit{booleans}$:
%
\begin{alignat*}{2}
  &\mathrlap{\textit{Booleans} : \square}\\
  &\textit{Booleans} = \record\{\ &&\ldots;\\
                                & &&\neg : \Bool \to \Bool\}
\end{alignat*}
%
\begin{alignat*}{2}
  &\mathrlap{\textit{booleans} : \textit{Booleans}}\\
  &\textit{booleans} = \{&&\ldots;\\
                      & &&\neg = \lambda b : \top + \top.\ \textit{case}\ b\ \textit{of}\\
                      & &&\ \ \ \ \ \ \ \ \ \ \inl\ () = \inr\ ()\\
                      & &&\ \ \ \ \ \ \ \ \ \ \inr\ () = \inl\ ()\}
\end{alignat*}
%
If we try to prove the same monotonicity theorem, that now shouldn't hold, we run into
issues when we try to provide $R_\neg$ in $R_{imp}$.
%
Specifically, the proof obligation for (i.e. type of) $R_\neg$ is the following:
%
\begin{alignat*}{2}
  R_\neg &\ :&&\  (b_0\ b_1 : \top + \top)\\
          &\to&&\ (R_b : b_0 \implies b_1)\\
          &\to&&\ \neg b_0 \implies \neg b_1
\end{alignat*}
%
Which clearly cannot be satisfied.

%% The key point is that a type can be interpreted\ch{unclear to me what you mean
%%   by ``interpreted'' here, which makes understanding the rest hard; in fact
%%   didn't get much of the rest of this section}
%% by \emph{any relation}, as long
%% as the operations manipulating this type involved can be given a compatible
%% interpretation.
%% %
%% Using the module structure is particularly useful here.\ch{here were?
%%   in this paper?}
%% 
%% Indeed, we could, say, interpret\ch{ditto}
%% the $sec$ module as $\rel{sec}$, but then we
%% would get rather uninformative interpretations for the modules depending on it
%% ($\rel{temp}\ sec\ sec\ \rel{sec}$).
%% %
%% Rather, we have the opportunity to define \emph{another}, more useful witness
%% of $R_{sec} : \rel{\Multef}\ sec\ sec$, which yields useful theorems about
%% clients.
%% %
%% In fact, in \cref{sec:transparency} we will go beyond and relate several
%% implementations of the $\Multef$ library.


==> texdirectives.tex <==
\draftfalse\anonfalse\camerafalse

